Conflict-Based Search for Multi-Agent Path Finding Among Movable Obstacles

This paper investigates Multi-Agent Path Finding Among Movable Obstacles (M-PAMO), which seeks collision-free paths for multiple agents from their start to goal locations among static and movable obstacles. M-PAMO arises in logistics and warehouses where mobile robots are among unexpected movable objects. Although Multi-Agent Path Finding (MAPF) and single-agent Path planning Among Movable Obstacles (PAMO) were both studied, M-PAMO remains under-explored. Movable obstacles lead to new fundamental challenges as the state space, which includes both agents and movable obstacles, grows exponentially with respect to the number of agents and movable obstacles. In particular, movable obstacles often closely couple agents together spatially and temporally. This paper makes a first attempt to adapt and fuse the popular Conflict-Based Search (CBS) for MAPF, and a recent single-agent PAMO planner called PAMO*, together to address M-PAMO. We compare their performance with up to 20 agents and hundreds of movable obstacles, and show the pros and cons of these approaches. Finally, we deploy our planner on real robots among movable obstacles in a lab setting, where the robots can push the movable obstacles in correct orders to reach their respective goals, which is otherwise hard to achieve with existing methods.

==> alg.tex <==
\setcounter{topnumber}{8}
\setcounter{bottomnumber}{8}
\setcounter{totalnumber}{8}

\begin{algorithm}[t]
\small
    \caption{Pseudocode for \abbrDMS}\label{dms:alg:dms}
    \begin{algorithmic}[1]
    %
    \State{$l_o \gets (v_o, \Vec{a}=0^M, \Vec{g}=0^N)$}\label{dms:alg:dms:lineInitBegin}
    \State{$parent(l_o) \gets NULL$, $f_{temp}(l_o) \gets 0$}
    
    \State{add $l_o$ to OPEN with $f_{temp}(l_o)$ as the priority}\label{dms:alg:dms:lineInitEnd}
    \State{add $l_o$ to $\FrontierSet(v_o)$}
    
    \While{OPEN is not empty} \label{dms:alg:dms:lineWhileBegin}
    
    
    \State{$l=(v,\Vec{a},\Vec{g}) \gets$ OPEN.pop() }

    \State{\procName{TargetSeq}($parent(l)$, $l$, $I_C(parent(l))$)}\label{dms:alg:dms:lineTargetSeq}
    \State{$f_{max}(l) \gets \max_{i\in I} \{ \vec{g}(l) +  w \cdot \vec{h}(l)$\} }\label{dms:alg:dms:lineFmax}
    \If{$f_{max}(l) > f_{temp}(l)$}\label{dms:alg:dms:lineFmaxCheck}
    \State{$f_{temp}(l) \gets f_{max}(l)$}
    \State{add $l$ to OPEN with $f_{temp}(l)$ as the priority}
    \State{\textbf{continue}}
    \EndIf

    \State{\textbf{if} $\procName{CheckSuccess}(l)$  \textbf{then}}
    \State{\indent \textbf{return} \procName{Reconstruct}($l$)}
    
    %		\State{move $s_k$ from OPEN($v_k$) to CLOSED($v_k$)}
    \State{$L_{succ} \gets$ \textsl{GetSuccessors}($l$) } 
    \ForAll{$l' \in L_{succ}$}
    
    \State{$I_C(l') \gets \procName{CheckConflict}(v(l),v(l'))$}\label{dms:alg:dms:lineDetectConflict}
    \State{\procName{BackProp}($l$, $I_C(l')$)}
    \If{$I_C \neq \emptyset$ \textbf{continue}}
    \EndIf
    
    \If{\procName{IsDominated}($l'$)}
    \State{\procName{DomBackProp($l,l'$)}}
    \State{\textbf{continue}}
    \EndIf
    
    \State{$f_{temp}(l') \gets \max_{i\in I} \{ \Vec{g}(l') + w \cdot \procName{SimpleHeu}(l') \}$}\label{dms:alg:dms:lineGetF}
    \State{$parent(l') \gets l$}
    \State{add $l'$ to $\FrontierSet(v(l'))$ and back\_set($l'$)}
    \State{add $l'$ OPEN with $f_{temp}(l')$ as the priority}
    \EndFor
    \EndWhile \label{dms:alg:dms:lineWhileEnd}
    \State{\textbf{return} Failure (no solution)}
    \end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
\small
\caption{Pseudocode for \procName{TargetSeq}($l$, $l'$, $I_C(l)$)}\label{dms:alg:targetSeq}
\begin{algorithmic}[1]
    % \Statex{INPUT: two labels $l,l'$ where $l$ is the parent of $l'$.}
    \If{$l'$ is on-policy}
    \State{$\gamma(l') \gets \gamma(l)$, \textbf{return}}
    \EndIf

    \State{$\gamma(l') \gets \gamma(l)$}\label{dms:alg:targetSeq:lineCopySeq}
    \State{Compute $\phi_{\gamma(l')}$ and $\Vec{h}(l')$ based on $\gamma(l')$}\label{dms:alg:targetSeq:lineCopySeqThen}
    
    \If{$\exists i \in I_C(l), g^i(l') + h^i(l') > f_{max}(l')$}\label{dms:alg:targetSeq:lineCheckFmax}
    \State{$\gamma(l'),\Vec{h}(l'),\phi_{\gamma(l')} \gets \procName{SolveMHPP}(l')$}\label{dms:alg:targetSeq:lineCheckFmaxEnter}
    \EndIf
    \State{\textbf{return}}
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
\small
\caption{Pseudocode for BackProp($l,I_C(l')$)}\label{dms:alg:backprop}
\begin{algorithmic}[1]
    \If{$I_C(l') \nsubseteq I_C(l)$}
    \State{$I_C(l) \gets I_C(l') \bigcup I_C(l)$}
    \If{$l \notin$ OPEN}{ add $l$ to OPEN}
    \EndIf
    \ForAll{$l'' \in$ back\_set($l$)}
    \State{\procName{BackProp}($l''$, $I_C(l)$)}\label{dms:alg:backprop:lineRecursive}\label{dms:alg:backprop:lineKBPDecrease}
    \EndFor
    \EndIf
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\small
\caption{Pseudocode for DomBackProp($l,l'$)}\label{dms:alg:dom_back_prop}
\begin{algorithmic}[1]
    \ForAll{$l'' \in \FrontierSet(v(l'))$}
    \If{$l'' \succeq_l l' \text{ or } l'' = l'$}
    \State{\procName{BackProp}($l$, $I_C(l'')$)}
    \State{add $l$ to back\_set($l''$)}
    \EndIf
    \EndFor
\end{algorithmic}
\end{algorithm}



